Improving Anytime Prediction with Parallel Cascaded Networks and a Temporal-Difference Loss

Although deep feedforward neural networks share some characteristics with the primate visual system, a key distinction is their dynamics. Deep nets typically operate in serial stages wherein each layer completes its computation before processing begins in subsequent layers. In contrast, biological systems have cascaded dynamics: information propagates from neurons at all layers in parallel but transmission occurs gradually over time, leading to speed-accuracy trade offs even in feedforward architectures. We explore the consequences of biologically inspired parallel hardware by constructing cascaded ResNets in which each residual block has propagation delays but all blocks update in parallel in a stateful manner. Because information transmitted through skip connections avoids delays, the functional depth of the architecture increases over time, yielding anytime predictions that improve with internal-processing time. We introduce a temporal-difference training loss that achieves a strictly superior speed-accuracy profile over standard losses and enables the cascaded architecture to outperform state-of-the-art anytime-prediction methods. The cascaded architecture has intriguing properties, including: it classifies typical instances more rapidly than atypical instances; it is more robust to both persistent and transient noise than is a conventional ResNet; and its time-varying output trace provides a signal that can be exploited to improve information processing and inference.

==> err <==
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18>
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/article.cls
Document Class: article 2020/04/10 v1.4m Standard LaTeX document class
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/size10.clo))
(./neurips_2021.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/environ/environ.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(./natbib.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty))))
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/local/texlive/2021/texmf-dist/tex/latex/subfigure/subfigure.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/sidecap/sidecap.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/lm/lmodern.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/slantsc/slantsc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/lm/ot1lmr.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./main.aux (./appendix.aux))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
*geometry* verbose mode - [ preamble ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(92.14519pt, 430.00462pt, 92.14519pt)
* v-part:(T,H,B)=(95.39737pt, 556.47656pt, 143.09605pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=430.00462pt
* \textheight=556.47656pt
* \oddsidemargin=19.8752pt
* \evensidemargin=19.8752pt
* \topmargin=-13.87262pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

*geometry* verbose mode - [ newgeometry ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(108.405pt, 397.48499pt, 108.40501pt)
* v-part:(T,H,B)=(72.26999pt, 650.43pt, 72.27pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=397.48499pt
* \textheight=650.43pt
* \oddsidemargin=36.13501pt
* \evensidemargin=36.13501pt
* \topmargin=-37.0pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/ragged2e/ragged2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/everysel/everysel.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/everysel/everysel-2011-10-28.sty
ABD: EverySelectfont initializing macros)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./main.out) (./main.out)
(/usr/local/texlive/2021/texmf-dist/tex/latex/lm/omllmm.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/lm/omslmsy.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/lm/omxlmex.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/microtype/mt-msb.cfg) [1{/usr/loc
al/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
(/usr/local/texlive/2021/texmf-dist/tex/latex/lm/ts1lmr.fd)
Underfull \vbox (badness 10000) has occurred while \output is active [2]
[3 <./fig1_Combined.pdf>] [4 <./example.pdf>]
(/usr/local/texlive/2021/texmf-dist/tex/latex/lm/ot1lmtt.fd) [5 <./varyingTDlam
bda.pdf>] (/usr/local/texlive/2021/texmf-dist/tex/latex/lm/omslmr.fd) [6 <./Spe
edAccuracy_rightlegend.pdf>] [7 <./TaxonomicCompliance.pdf>]
Underfull \vbox (badness 2221) has occurred while \output is active [8 <./Noise
Types4.pdf>] [9 <./metacog_ood.pdf>] (./main.bbl [10] [11] [12]
Underfull \hbox (badness 1178) in paragraph at lines 297--300
[]\OT1/lmr/m/n/10 (+20) S. Zagoruyko and N. Ko-modakis.  Wide resid-ual net-wor
ks.  \OT1/lmr/m/it/10 (+20) arXiv preprint
) [13] [14] (./appendix.tex [15]

LaTeX Font Warning: Font shape `OT1/lmr/bx/sc' undefined
(Font)              using `OT1/lmr/bx/n' instead on input line 102.

[16] [17 <./stationary_noise_types.pdf> <./speed_acc_tradeoff_gt.pdf

pdfTeX warning: pdflatex (file ./speed_acc_tradeoff_gt.pdf): PDF inclusion: mul
tiple pdfs with page group included in a single page
>]
Underfull \vbox (badness 1622) has occurred while \output is active [18 <./Seri
alTD01.pdf> <./cifar10_samples__cascaded_TD.pdf> <./cifar10_samples__cascaded_S
EQ.pdf

pdfTeX warning: pdflatex (file ./cifar10_samples__cascaded_SEQ.pdf): PDF inclus
ion: multiple pdfs with page group included in a single page
>]
! Too many }'s.
l.293 ...ss subset of ImageNet \{deng2009imagenet}
                                                   and it contains 10,000 va...

? Type <return> to proceed, S to scroll future error messages,
R to run without stopping, Q to run quietly,
I to insert something, E to edit your file,
1 or ... or 9 to ignore the next 1 to 9 tokens of input,
H for help, X to quit.
? ! Too many }'s.
l.295 ... Scene UNderstanding (LSUN) \{yu2015lsun}
                                                   consists of 10 scenes cat...

? ! Too many }'s.
l.297 ...House Numbers (SVHN) \{netzer2011reading}
                                                   dataset is obtained from ...

? ! Too many }'s.
l.302 ...remove random variance \{masson2003using}
                                                  .
? ! Interruption.
<to be read again> 
                   .
l.302 ...emove random variance \{masson2003using}.
                                                  
? ! Too many }'s.
l.304 ...d resize variations \{liang2017enhancing}
                                                   to
? [19]) [20 <./CascadedTD__rnn__gru__cascadedTD__with_labels.pdf> <./cascaded_seq
_metacog.pdf

pdfTeX warning: pdflatex (file ./cascaded_seq_metacog.pdf): PDF inclusion: mult
iple pdfs with page group included in a single page
>] (./main.aux (./appendix.aux))

LaTeX Font Warning: Some font shapes were not available, defaults substituted.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 ){/usr/local/texlive/2021/texmf-dist/fonts/enc/dvips/lm/lm-rm.enc}{/usr/local/
texlive/2021/texmf-dist/fonts/enc/dvips/lm/lm-mathsy.enc}{/usr/local/texlive/20
21/texmf-dist/fonts/enc/dvips/lm/lm-rmtt.enc}{/usr/local/texlive/2021/texmf-dis
t/fonts/enc/dvips/lm/lm-mathit.enc}{/usr/local/texlive/2021/texmf-dist/fonts/en
c/dvips/lm/lm-mathex.enc}{/usr/local/texlive/2021/texmf-dist/fonts/enc/dvips/lm
/lm-rmsc.enc}{/usr/local/texlive/2021/texmf-dist/fonts/enc/dvips/lm/lm-ts1.enc}
</usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb><
/usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmcsc10.pfb><
/usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></
usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmmib10.pfb></
usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmr17.pfb></us
r/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmss17.pfb></usr
/local/texlive/2021/texmf-dist/fonts/type1/public/lm/lmbx10.pfb></usr/local/tex
live/2021/texmf-dist/fonts/type1/public/lm/lmbx12.pfb></usr/local/texlive/2021/
texmf-dist/fonts/type1/public/lm/lmbx7.pfb></usr/local/texlive/2021/texmf-dist/
fonts/type1/public/lm/lmbx9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/lm/lmcsc10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/l
m/lmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/lm/lmmi10.p
fb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/lm/lmmi7.pfb></usr/lo
cal/texlive/2021/texmf-dist/fonts/type1/public/lm/lmmi9.pfb></usr/local/texlive
/2021/texmf-dist/fonts/type1/public/lm/lmr10.pfb></usr/local/texlive/2021/texmf
-dist/fonts/type1/public/lm/lmr6.pfb></usr/local/texlive/2021/texmf-dist/fonts/
type1/public/lm/lmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/lm/lmr9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/lm/lmri10.p
fb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/lm/lmri9.pfb></usr/lo
cal/texlive/2021/texmf-dist/fonts/type1/public/lm/lmsy10.pfb></usr/local/texliv
e/2021/texmf-dist/fonts/type1/public/lm/lmsy5.pfb></usr/local/texlive/2021/texm
f-dist/fonts/type1/public/lm/lmsy6.pfb></usr/local/texlive/2021/texmf-dist/font
s/type1/public/lm/lmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pub
lic/lm/lmsy9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/lm/lmtt
10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfonts/symbols/
msbm10.pfb>
Output written on main.pdf (20 pages, 3962279 bytes).
Transcript written on main.log.

